Smooth Quasar-Convex Optimization with Constraints

Quasar-convex functions form a broad nonconvex class with applications to linear dynamical systems, generalized linear models, and Riemannian optimization, among others. Current nearly optimal algorithms work only in affine spaces due to the loss of one degree of freedom when working with general convex constraints. Obtaining an accelerated algorithm that makes nearly optimal $\widetilde{O}(1/(\gamma\sqrt{\varepsilon}))$ first-order queries to a $\gamma$-quasar convex smooth function \emph{with constraints} was independently asked as an open problem in Mart\'inez-Rubio (2022); Lezane, Langer, and Koolen (2024). In this work, we solve this question by designing an inexact accelerated proximal point algorithm that we implement using a first-order method achieving the aforementioned rate and, as a consequence, we improve the complexity of the accelerated geodesically Riemannian optimization solution in Mart\'inez-Rubio (2022). We also analyze projected gradient descent and Frank-Wolfe algorithms in this constrained quasar-convex setting. To the best of our knowledge, our work provides the first analyses of first-order methods for quasar-convex smooth functions with general convex constraints.

==> includes/definitions.tex <==
%
\usepackage{xparse}
\usepackage{xargs}

\makeatletter %
\def\Hy@raisedlink@left#1{%
    \ifvmode
        #1%
    \else
        \Hy@SaveSpaceFactor
        \llap{\smash{%
        \begingroup
            \let\HyperRaiseLinkLength\@tempdima
            \setlength\HyperRaiseLinkLength\HyperRaiseLinkDefault
            \HyperRaiseLinkHook
        \expandafter\endgroup
        \expandafter\raise\the\HyperRaiseLinkLength\hbox{%
            \Hy@RestoreSpaceFactor
            #1%
            \Hy@SaveSpaceFactor
        }%
        }}%
        \Hy@RestoreSpaceFactor
        \penalty\@M\hskip\z@ 
    \fi
}
\makeatother

\newcommand\newlink[2]{{\protect\hyperlink{#1}{\normalcolor #2}}}
\makeatletter
\newcommand\newtarget[2]{\Hy@raisedlink@left{\hypertarget{#1}{}}#2} %
%
\makeatother

%
%

\newcommand\linktoproof[1]{{\normalfont[{\hyperlink{proof:#1}{$\downarrow$}}]}}
%
%
\newcommand\linkofproof[1]{(\cref{#1}) \newtarget{proof:#1}}

%
\usepackage[bb=boondox]{mathalpha} %
%
\newcommand{\zeros}{\mathbb{0}} 
\newcommand\Hess{\operatorname{Hess}}

%
%
\newcommand{\PGD}{\newlink{def:acronym_projected_gradient_descent}{PGD}}
\newcommand{\GLM}{\newlink{def:acronym_generalized_linear_model}{GLM}}


\newcommand{\bigo}[1]{O( #1 )}
\newcommand{\bigol}[1]{O\left( #1 \right)}
\newcommand{\bigotilde}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}( #1 )}
\newcommand{\bigthetatilde}[1]{\newlink{def:big_o_tilde}{\widetilde{\Theta}}( #1 )}
\newcommand{\bigthetatildel}[1]{\newlink{def:big_o_tilde}{\widetilde{\Theta}}\left( #1 \right)}
\newcommand{\bigotildel}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}\left( #1 \right)}
\newcommand{\bigomegatilde}[1]{\newlink{def:big_o_tilde}{\widetilde{\Omega}}( #1 )}

\newcommand{\return}{\textbf{return}}

\newcommand{\psix}{\psi_{\texttt x}}
\newcommand{\psiy}{\psi_{\texttt y}}


\newcommand{\Y}{\mathcal{Y}}


\newcommand\set[1]{\{ #1 \}}
\newcommand\setl[1]{\left\{ #1 \right\}}
\newcommand\setsuch[2]{\{ #1 \mid #2  \}}
\newcommand\setsuchl[2]{\left\{ #1 \mid #2  \right\}}



\newcommandx*\prox[1][1=\lambda, usedefault]{\newlink{def:prox_point}{\operatorname{prox}}_{#1}}
\renewcommandx*\M[1][1=, usedefault]{\newlink{def:Moreau_Yoshida_envelope}{M_{#1}}}



\renewcommand\dim{\newlink{def:dimension}{d}} 
\newcommand\Rd{\R^{\dim}} 

\newcommand\dom{\operatorname{dom}}
\newcommand\diam{\operatorname{diam}}

\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\newlink{def:accuracy_epsilon}{\oldepsilon}}

\newcommand\tildeepsilon{\newlink{def:binary_search_accuracy}{\tilde{\oldepsilon}}}


\let\oldgamma\gamma
\renewcommand{\gamma}{\newlink{def:quasar_convexity_constant}{\oldgamma}}

\let\oldmu\mu
\renewcommand{\mu}{\newlink{def:strong_convexity}{\oldmu}}

\let\oldlambda\lambda
\renewcommand{\lambda}{\newlink{def:moreau_regularization_parameter}{\oldlambda}}

\usepackage{cancel}
%
\newcommand\Ccancel[2][black]{
    \let\OldcancelColor\CancelColor
    \renewcommand\CancelColor{\color{#1}}
    \cancel{#2}
    \renewcommand\CancelColor{\OldcancelColor}
}

\newcommand\Cbcancel[2][black]{
    \let\OldcancelColor\CancelColor
    \renewcommand\CancelColor{\color{#1}}
    \bcancel{#2}
    \renewcommand\CancelColor{\OldcancelColor}
}


\newcommand\indicator[1]{\newlink{def:set_indicator}{\mathbf{1}_{#1}}}

\newcommand\eventindicator[1]{\newlink{def:event_indicator_function}{\mathbb{I}}(#1)}

\newcommandx*\argmindelta[2][1=, 2=\delta, usedefault]{\newlink{def:approximate_argmin}{\argmin_{#1}^{#2}}}

\newcommandx*\gradmtilde[1][1=, usedefault]{\newlink{def:approximate_gradient_of_moreau_envelope}{\widetilde{\nabla} M_{#1}}}


\newcommandx*\mtilde[1][1=, usedefault]{\newlink{def:approximate_moreau_envelope}{\widetilde{M}_{#1}}}

\newcommand\conv[1]{\newlink{def:convex_combination}{\operatorname{conv}}\set{#1}}
\newcommand\proj[1]{\newlink{def:projection_operator}{\operatorname{Proj}}_{#1}}

\newcommand\gradmap[1]{\newlink{def:gradient_mapping}{g_{#1}}}

\let\strikedL\L
\renewcommand{\L}{\newlink{def:smoothness_constant}{L}} 

\newcommand{\Ltilde}{\newlink{def:some_other_smoothness_constant}{\widetilde{L}}} 
\newcommand{\Lhat}{\newlink{def:smoothness_for_the_line_problem}{\hat{L}}} 
\newcommand{\mutilde}{\newlink{def:some_other_str_convexity_constant}{\widetilde{\mu}}} 

\newcommand{\valpha}{\newlink{def:intermediate_point_in_line_search}{v_\alpha}} 
\newcommand{\walpha}{\newlink{def:prox_of_v_alpha}{w_\alpha}} 
%

\renewcommand\D{\newlink{def:diameter_of_feasible_set}{D}}
\newcommand\X{\newlink{def:feasible_set}{\mathcal{X}}}


